Nearest Neighbour Decoding and Pilot-Aided Channel Estimation in Stationary Gaussian Flat-Fading Channels

We study the information rates of non-coherent, stationary, Gaussian, multiple-input multiple-output (MIMO) flat-fading channels that are achievable with nearest neighbour decoding and pilot-aided channel estimation. In particular, we analyse the behaviour of these achievable rates in the limit as the signal-to-noise ratio (SNR) tends to infinity. We demonstrate that nearest neighbour decoding and pilot-aided channel estimation achieves the capacity pre-log - which is defined as the limiting ratio of the capacity to the logarithm of SNR as the SNR tends to infinity - of non-coherent multiple-input single-output (MISO) flat-fading channels, and it achieves the best so far known lower bound on the capacity pre-log of non-coherent MIMO flat-fading channels.

==> extra_2T_transmission.tex <==
\begin{pspicture}(-1,-2)(14,2)

{

\rput(1,0.15){\scriptsize $t = 1$}

\rput(2.9,0.7){\scriptsize $L(T-1)$}
\psline[linewidth=0.02,linestyle=dotted,dotsep=1pt]{<->}(1.8,0.5)(4,0.5)

\psframe[linewidth=0.02,fillstyle=hlines](4,0)(8.5,0.3)


\psframe[linewidth=0.02](2.9,0)(3.5,0.3)
\psframe[linewidth=0.02,fillstyle=solid,fillcolor=darkgray](2.9,0)(3.2,0.3)

\psframe[linewidth=0.02](1.8,0)(2.4,0.3)
\psframe[linewidth=0.02,fillstyle=solid,fillcolor=darkgray](1.8,0)(2.1,0.3)

\psframe[linewidth=0.02](9,0)(9.6,0.3)
\psframe[linewidth=0.02,fillstyle=solid,fillcolor=darkgray](9,0)(9.3,0.3)

\psframe[linewidth=0.02](10.1,0)(10.7,0.3)
\psframe[linewidth=0.02,fillstyle=solid,fillcolor=darkgray](10.1,0)(10.4,0.3)

}

\rput(6.25,-1){\scriptsize $N$}
\psline[linewidth=0.02,linestyle=dotted,dotsep=1pt]{<->}(4,-0.8)(8.5,-0.8)

{

\rput(1,-0.45){\scriptsize $t = 2$}

\rput(9.6,0.7){\scriptsize $L(T-1)$}
\psline[linewidth=0.02,linestyle=dotted,dotsep=1pt]{<->}(8.5,0.5)(10.7,0.5)

\psframe[linewidth=0.02,fillstyle=hlines](4,-0.6)(8.5,-0.3)

\psframe[linewidth=0.02](2.9,-0.6)(3.5,-0.3)
\psframe[linewidth=0.02,fillstyle=solid,fillcolor=darkgray](3.2,-0.6)(3.5,-0.3)

\psframe[linewidth=0.02](1.8,-0.6)(2.4,-0.3)
\psframe[linewidth=0.02,fillstyle=solid,fillcolor=darkgray](2.1,-0.6)(2.4,-0.3)

\psframe[linewidth=0.02](9,-0.6)(9.6,-0.3)
\psframe[linewidth=0.02,fillstyle=solid,fillcolor=darkgray](9.3,-0.6)(9.6,-0.3)

\psframe[linewidth=0.02](10.1,-0.6)(10.7,-0.3)
\psframe[linewidth=0.02,fillstyle=solid,fillcolor=darkgray](10.4,-0.6)(10.7,-0.3)

}

\end{pspicture}

==> one_block_estimation.tex <==
%%% A data block estimation
\begin{pspicture}(-1.3,-2)(14,2)

\rput(3,0.7){\scriptsize $L(T-1)$}
\psline[linewidth=0.02,linestyle=dotted,dotsep=1pt]{<->}(1.4,0.5)(4.6,0.5)

\rput(8.9,0.7){\scriptsize $L(T-1)$}
\psline[linewidth=0.02,linestyle=dotted,dotsep=1pt]{<->}(7.3,0.5)(10.5,0.5)

{
\rput(0.5,0.15){\scriptsize $t=1$}
\psframe[linewidth=0.02](4.6,0)(7.3,0.3)
\psframe[linewidth=0.02,fillstyle=solid,fillcolor=darkgray](4.6,0)(4.9,0.3)
\psframe[linewidth=0.02,fillstyle=solid,fillcolor=lightgray](5.2,0)(6.7,0.3)
\psframe[linewidth=0.02,fillstyle=solid,fillcolor=darkgray](6.7,0)(7,0.3)

\psframe[linewidth=0.02](1.4,0)(2,0.3)
\psframe[linewidth=0.02,fillstyle=solid,fillcolor=darkgray](1.4,0)(1.7,0.3)
\rput(2.5,0.15){$\dotsc$}

\psframe[linewidth=0.02](3,0)(3.6,0.3)
\psframe[linewidth=0.02,fillstyle=solid,fillcolor=darkgray](3,0)(3.3,0.3)
\rput(4.1,0.15){$\dotsc$}

\rput(7.8,0.15){$\dotsc$}
\psframe[linewidth=0.02](8.3,0)(8.9,0.3)
\psframe[linewidth=0.02,fillstyle=solid,fillcolor=darkgray](8.3,0)(8.6,0.3)
\rput(9.4,0.15){$\dotsc$}

\psframe[linewidth=0.02](9.9,0)(10.5,0.3)
\psframe[linewidth=0.02,fillstyle=solid,fillcolor=darkgray](9.9,0)(10.2,0.3)

{
\psline[linewidth=0.02](5.5,0)(5.5,0.3)
\psline[linewidth=0.02](5.8,0)(5.8,0.3)
\psline[linewidth=0.02](6.1,0)(6.1,0.3)
\psline[linewidth=0.02](6.4,0)(6.4,0.3)
}
}

{
\rput(0.5,-0.45){\scriptsize $t=2$}
\psframe[linewidth=0.02](4.6,-0.6)(7.3,-0.3)
\psframe[linewidth=0.02,fillstyle=solid,fillcolor=darkgray](4.9,-0.6)(5.2,-0.3)
\psframe[linewidth=0.02,fillstyle=solid,fillcolor=lightgray](5.2,-0.6)(6.7,-0.3)
\psframe[linewidth=0.02,fillstyle=solid,fillcolor=darkgray](7,-0.6)(7.3,-0.3)

\psframe[linewidth=0.02](1.4,-0.6)(2,-0.3)
\psframe[linewidth=0.02,fillstyle=solid,fillcolor=darkgray](1.7,-0.6)(2,-0.3)
\rput(2.5,-0.45){$\dotsc$}

\psframe[linewidth=0.02](3,-0.6)(3.6,-0.3)
\psframe[linewidth=0.02,fillstyle=solid,fillcolor=darkgray](3.3,-0.6)(3.6,-0.3)
\rput(4.1,-0.45){$\dotsc$}

\rput(7.8,-0.45){$\dotsc$}
\psframe[linewidth=0.02](8.3,-0.6)(8.9,-0.3)
\psframe[linewidth=0.02,fillstyle=solid,fillcolor=darkgray](8.6,-0.6)(8.9,-0.3)
\rput(9.4,-0.45){$\dotsc$}

\psframe[linewidth=0.02](9.9,-0.6)(10.5,-0.3)
\psframe[linewidth=0.02,fillstyle=solid,fillcolor=darkgray](10.2,-0.6)(10.5,-0.3)

{
\psline[linewidth=0.02](5.5,-0.6)(5.5,-0.3)
\psline[linewidth=0.02](5.8,-0.6)(5.8,-0.3)
\psline[linewidth=0.02](6.1,-0.6)(6.1,-0.3)
\psline[linewidth=0.02](6.4,-0.6)(6.4,-0.3)
}

}

\rput(5.95,-1){\scriptsize $L - n_{\rm t}$}
\psline[linewidth=0.02,linestyle=dotted,dotsep=1pt]{<->}(5.2,-0.8)(6.7,-0.8)
\end{pspicture}

==> system_model.tex <==
%% System Model

\begin{pspicture}(1.5,-2)(14,2)
\small 
\rput(0,0){$m$} 
\psline[linewidth=0.03]{->}(0.25,0)(0.75,0)
\psframe[linewidth=0.04,dimen=outer](0.75,-0.5)(1.75,0.5)
\rput(1.25,0){ENC}

\psline[linewidth=0.03]{->}(1.75,0)(3,0)
\psframe[linewidth=0.04,dimen=outer](3,-0.6)(5,0.6)
\rput(4,0.25){Pilot}
\rput(4,-0.25){Insertion}

\psline[linewidth=0.03]{->}(5,0)(6,0)
\psframe[linewidth=0.04,dimen=outer](6,-0.5)(8,0.5)
\rput(7,0){Channel}

\psline[linewidth=0.03]{->}(8,0)(9,0)
\psframe[linewidth=0.04,dimen=outer](9,-0.7)(11,0.7)
\rput(10,0.35){Splitter}
\psline[linewidth=0.03cm](9.5,-0.3)(10,-0.3)
\psline[linewidth=0.03cm](10,-0.3)(10.5,-0.1)
\psline[linewidth=0.03cm](10,-0.3)(10.5,-0.5)
\psline[linewidth=0.03]{->}(11,0.7)(12,1)
\psline[linewidth=0.03]{->}(11,-0.7)(12,-1)

\psframe[linewidth=0.04,dimen=outer](12,1)(14,2.2)
\rput(13,1.8){Channel}
\rput(13,1.4){Estimator}
\psline[linewidth=0.03]{->}(13,1)(13,-1)

\psframe[linewidth=0.04,dimen=outer](12,-1)(14,-2)
\rput(13,-1.5){DEC}

\psline[linewidth=0.03]{->}(14,-1,0)(15,-0.2)
\rput(15,0){$\hat m$}

\end{pspicture}
